DFlow: Efficient Dataflow-based Invocation Workflow Execution for Function-as-a-Service

The Serverless Computing is becoming increasingly popular due to its ease of use and fine-grained billing. These features make it appealing for stateful application or serverless workflow. However, current serverless workflow systems utilize a controlflow-based invocation pattern to invoke functions. In this execution pattern, the function invocation depends on the state of the function. A function can only begin executing once all its precursor functions have completed. As a result, this pattern may potentially lead to longer end-to-end execution time. We design and implement the DFlow, a novel dataflow-based serverless workflow system that achieves high performance for serverless workflow. DFlow introduces a distributed scheduler (DScheduler) by using the dataflow-based invocation pattern to invoke functions. In this pattern, the function invocation depends on the data dependency between functions. The function can start to execute even its precursor functions are still running. DFlow further features a distributed store (DStore) that utilizes effective fine-grained optimization techniques to eliminate function interaction, thereby enabling efficient data exchange. With the support of DScheduler and DStore, DFlow can achieving an average improvement of 60% over CFlow, 40% over FaaSFlow, 25% over FaasFlowRedis, and 40% over KNIX on 99%-ile latency respectively. Further, it can improve network bandwidth utilization by 2x-4x over CFlow and 1.5x-3x over FaaSFlow, FaaSFlowRedis and KNIX, respectively. DFlow effectively reduces the cold startup latency, achieving an average improvement of 5.6x over CFlow and 1.1x over FaaSFlow

==> Sec/limitation.tex <==
% \section{Limitations and Discussion }

% In this section, we discuss the advantages and several limitations of the DFlow.Compared to some existing controlflow-based serverless systems, such as FaaSFlow~\cite{FaaSFlow} and others, DFlow can invoke functions based on the data dependence with major module: 1) dataflow-based two-layer scheduler; 2) data directory service to separate the data and metadata; 3)fine-grained hierarchical pipeline distributed store. Together, they allow DFlow to support efficient workflow with low e2e latency and high throughput.

% Despite these advantages, the DFlow still has some limitations.
% \begin{itemize}
%     \item Compared to FaaSFlow~\cite{FaaSFlow}, DFlow consumes more memory because the DFlow uses the in-memory store for all function data transfer, while FaaSFlow~\cite{FaaSFlow} uses the CouchDB for remote data transfer.
%     \item Compared to Beldi~\cite{Beldi-OSDI20} and Boki~\cite{Boki-SOSP21}, DFlow does not support fault tolerance. 
%     \item Compared to Boki~\cite{Boki-SOSP21} that supports sequential consistency and Cloudburst~\cite{cloudburst} that supports casual consistency, the DStore only supports read consistency.  
    
% \end{itemize}
